Existence and Minimax Theorems for Adversarial Surrogate Risks in Binary Classification

Adversarial training is one of the most popular methods for training methods robust to adversarial attacks, however, it is not well-understood from a theoretical perspective. We prove and existence, regularity, and minimax theorems for adversarial surrogate risks. Our results explain some empirical observations on adversarial robustness from prior work and suggest new directions in algorithm development. Furthermore, our results extend previously known existence and minimax theorems for the adversarial classification risk to surrogate risks.

==> Sections/Dual_Existence.tex <==
\section{Dual Maximizers}\label{sec:dual_existence}

To prove Theorem~\ref{th:dual_existence}, we show that $\dl$ is upper semi-continuous on the space $\Wball \e(\PP_0)\times \Wball \e(\PP_1)$ with respect to the weak topology on probability measures and furthermore the $W_\infty$ ball is compact with respect to this notion of convergence. 

\subsection{The semi-continuity of $\dl$}
Recall that when proving Lemma~\ref{lemma:duality_compact}, the calculation of $\Xi^*(\PP_0',\PP_1')$ showed that if $\PP_0',\PP_1'$ are supported on the compact set $K$, then the functional $\Xi^*(\PP_0',\PP_1')$ can be written as the infimum of integals of functions in $C_b(K^\e)$ (see  Lemma~\ref{lemma:Xi_star}). We extend this lemma to distributions with unbounded support by approximation.

   
   
   We also use the following measurable selection theorem:



    We apply a portion of the Portmanteau theorem \cit{billingsley}
    \begin{theorem}\label{th:portmanteau}
        Assume that $\QQ^n$ converges weakly to $\QQ$. Then if $\QQ(\partial A)=0$, then $\lim_{n\to \infty} \QQ^n(A)=\QQ(A)$.
    \end{theorem}

    \begin{lemma}\label{lemma:weak_convergence_restriction}
    Let $\nu_n$ be a sequence of measures that converges to $\nu$. Let $K$ be a compact set. Then the sequence $\nu^n_K$ defined by $\nu^n_K(A)=\nu^n(A\cap K)$ converges weakly to $\nu_K$, where $\nu_K$ is given by $\nu(A)=\nu(A\cap K)$.
    \end{lemma}
    \begin{proof}
    \todo{}
    \end{proof}
    
    
\begin{lemma}\label{lemma:dl_upper_semicontinuous}
    The functional $\dl$ is concave and upper semi-continuous with respect to the weak topology of probability measures.
\end{lemma}
\begin{proof}
    Let $\QQ_0^n,\QQ_1^n$ be sequences of measures converging to $\QQ_0,\QQ_1$ respectively. Set $\QQ\colon =\QQ_0+\QQ_1$.
    
    The proof proceeds in three steps.
    \begin{enumerate}
    \item   
    Define a function $F(R)\colon= \QQ(\ov{B_R(\zero)}^C)$. Then because this function is non-increasing, it has finitely many points of discontinuity. 

    Let $\delta>0$ be arbitrary and choose $R$ large enough so that $F(R)<\delta$ and $F$ is continuous at $R$.
    
  

    \item Now let $\nu_0,\nu_1$ be arbitrary measures. Consider $\nu_i^n$ defined by 

    \begin{equation}\label{eq:nu_restriction}
        \nu_i^R=\nu_i(\Rset^d)\cdot \frac{\nu_i(A\cap \ov{B_R(\zero)})}{\nu_i(\ov{B_R(\zero)})}
    \end{equation}
    Set $\nu=\nu_0+\nu_1$, $\eta=d\nu_1/d\nu$.
    Then
    \begin{align}
    &|\dl(\nu_0^R,\nu_1^R)-\dl(\nu_0,\nu_1)|=\left| \int C_\phi^*(\eta)\nu(\Rset^d)\frac{\one_{\ov{B_R(\zero)}}}{\nu(\ov{B_R(\zero)})}d\nu- \int C_\phi^*(\eta)d\nu \right|\nonumber\\
    &=  \int \left|C_\phi^*(\eta)\left( \nu(\Rset^d)\frac{\one_{\ov{B_R(\zero)}}}{\nu(\ov{B_R(\zero)})}-1\right)\right|d\nu \leq C_\phi^*\left( \frac 12 \right)\left( \int \left(\frac{\nu(\Rset^d)}{\nu(\ov{B_R(\zero)})} -1 \right)\one_{\ov{B_R(\zero)}}d\nu +\int \|\one_{\ov{B_R(\zero)}}-1| d\nu\right)\nonumber\\
    &\leq 2 C_\phi^*\left(\frac 12 \right) \nu(\ov{B_R(\zero)}^C)\label{eq:bound_last}
    \end{align}
    \item 
    By Lemma~\ref{lemma:weak_convergence_restriction}, If we define $\QQ_{i,R},\QQ_{i,R}^n$ via $\QQ_{i,R}(A)=\QQ_i(A\cap \ov{B_R(\zero)}$,  $\QQ_{i,R}^n(A)=\QQ_i^n(A\cap \ov{B_R(\zero)}$, $\QQ_{i,R}^n$ converges weakly to $\QQ_{i,R}^n$. Thus by Lemma~\ref{lemma:Xi_star},
    \[\limsup_{n\to \infty} \dl(\QQ_{0,R}^n,\QQ_{1,R}^n)\leq \dl(\QQ_{0,R},\QQ_{1,R})\]
    Pick $N$ large enough so that $n>N$ will imply
    \begin{equation}\label{eq:usc_bound}
        \dl(\QQ_{0,R}^n,\QQ_{1,R}^n)\leq \delta+\dl(\QQ_{0,R},\QQ_{1,R})
    \end{equation}

    and $|\QQ^n(\ov{B_R(\zero)})-\QQ(\ov{B_R(\zero)})|<\delta$. (This second criterion is possible due to Theorem~\ref{th:portmanteau}. Then \eqref{eq:bound_last} implies that
    \begin{equation}\label{eq:restricted_bounds}
    |\dl(\QQ_{0,R}^n,\QQ_{1,R}^n)-\dl(\QQ_0^n,\QQ_1^n)|\leq 4C_\phi^*(1/2)\delta,\quad |\dl(\QQ_{0,R},\QQ_{1,R})-\dl(\QQ_0,\QQ_1)|\leq 2C_\phi^*(1/2)\delta
    \end{equation}
    The relations \eqref{eq:usc_bound} and \eqref{eq:restricted_bounds} imply that
    \[\dl(\QQ_0^n,\QQ_1^n)\leq (6C_\phi^*(1/2) +1)\delta +\dl(\QQ_0,\QQ_1)\]
    Because $\delta$ was arbitrary, this implies the result.
    \end{enumerate}
\end{proof}










\subsection{The Compactness of the $W_\infty$ ball}
Recall that the $\empty^\e$ operation was defined in \eqref{eq:e_operation_def}. The $W_\infty$ distance between two probability distributions can be expressed in terms of this operation.

\begin{restatable}{lem}{lemmaWinfsetcharacterization}\label{lemma:W_inf_set_characterization}
        Let $\PP,\QQ$ be two finite positive measures with $\PP(\Rset^d)=\QQ(\Rset^d)$.
     Then
     \begin{equation}\label{eq:W_inf_set_characterization}
         W_\infty(\PP,\QQ)=\inf \{\e\colon \PP(A)\leq \QQ(A^\e) \forall \text{ measurable } A\}%=\inf \{\e\colon \PP(A)\leq \QQ(A^\e) \forall \text{ closed } A\}
     \end{equation}
\end{restatable}

Notice that this result is the analog of Lemma~\ref{lemma:W_inf_integral_characterization} for indicator functions.We prove Lemma~\ref{lemma:W_inf_set_characterization} in Appendix~\ref{app:W_infty}.


The topology of weak convergence is in fact metrizable, and Lemma~\ref{lemma:W_inf_set_characterization} provides a convenient comparison with this metrix. We will prove compactness by comparing a metric that metrizes the weak topology with the $W_\infty$ distance.
\begin{definition}
    The Levy-Prokhorov metric between two probability measures is defined by 
    \begin{equation}\label{eq:levy_prokhorov}
        d_\pi(\rho,\nu)=\inf\{ \e \colon \rho(A)\leq \nu(A\oplus B_\e(\zero))+\e \text{ and }\nu(A)\leq \rho (A\oplus B_\e(\zero))+\e\text{ for all Borel }A\}
    \end{equation}
    Let $\cB^\pi_\e(\PP)=\{\QQ\colon d_\pi(\PP,\QQ)\leq \e\}$
\end{definition}
\todo{make that $B$ bold, $\pi$ with $d_\pi$}
Because $\ov{B_\e(\zero)}\supset B_\e(\zero)=\bigcup_{\delta<\e} \ov{B_\delta(\zero)}$, one can in fact conclude
\[d_\pi(\rho,\nu)=\inf\{ \e \colon \rho(A)\leq \nu(A^\e)+\e\text{ and }\nu(A)\leq \rho(A^\e)+\e \text{ for all Borel }A\}\]
where the values of $\rho(A^\e), \nu(A^\e)$ are defined via their completion.
\begin{theorem}\label{th:levy_prokhorov_metrizability}
    The Levy-Prokhorov metric metrizes convergence with respect to the weak topology on probability measures.
\end{theorem}
This result is Theorem~6.8 of \citep{BillingsleyConvergenceOfProbabilityMeasures}.

The formula \eqref{eq:levy_prokhorov} provides an easy comparison between the $d_\pi$ and $W_\infty$ due to Lemma~\ref{lemma:W_inf_set_characterization}.

 Finally, we show compactness of the $W_\infty$ ball.
\begin{lemma}\label{lemma:W_infty_ball_weakly_compact}
    The $W_\infty$ ball is compact with respect to the topology of weak convergence of probability measures.
\end{lemma}



\begin{proof}
    We first show that for any two Borel measures, $d_\pi(\nu,\rho)\leq W_\infty(\nu,\rho)$. By \eqref{eq:levy_prokhorov}
     \begin{align*}
     &d_\pi(\rho,\nu)=\inf\{ \e \colon \rho(A)\leq \nu(A^\e)+\e\text{ and }\nu(A)\leq \rho(A^\e)+\e \text{ for all Borel }A\}\\
     &\leq \inf\{ \e \colon \rho(A)\leq \nu(A^\e)\} =W_\infty(\rho,\nu)&\text{(Lemma~\ref{lemma:W_inf_set_characterization})}
 \end{align*}
    
    Thus $\Wball \e( \nu)\subset \cB_\e^\pi(\nu)$. Thus if $\QQ_i$ is a sequence of measures in $\Wball \e (\nu)$, there is a subsequence $\QQ_{i_j}$ that weakly converges to a measure $\QQ$. It remains to show that $\QQ\in \Wball \e (\nu)$. By Lemma~\ref{lemma:W_inf_integral_characterization}
    \[\int S_\e(h)d\nu\geq \int h d\QQ_i\] for all bounded continuous $h$. By taking a limit, we can conclude that
    \[\int S_\e(h)d\nu\geq \int h d\QQ\] for all bounded continuous $h$. Lemma~\ref{lemma:W_inf_integral_characterization} then implies that $\QQ\in \Wball \e (\nu)$.
\end{proof}

Lastly, Lemmas~\ref{lemma:dl_upper_semicontinuous} and~\ref{lemma:W_infty_ball_weakly_compact} prove the existence of maximizers to the dual.

\thdualexistence*
\begin{proof}
Let $(\PP_0^n,\PP_1^n)$ be a sequence that minimizes $\dl$ over $\Wball \e(\PP_0)\Wball \e (\PP_1)$. Because the space $\Wball \e(\PP_0)\times \Wball \e(\PP_1)$ is weakly compact, there is a weakly convergent subsequence $(\PP_0^{n_k},\PP_1^{n_k})$. Define 
\[\PP_0^*=\lim_{k\to\infty} \PP_0^{n_k}\text{ and }\PP_1^*=\lim_{k\to \infty}\PP_1^{n_k}
\]
Then because $\dl$ is upper semi-continuous (Lemma~\ref{lemma:W_infty_ball_weakly_compact}), one can conclude that 
\[\lim_{k\to \infty}\dl(\PP_0^{n_k},\PP_1^{n_k})\leq \dl(\PP_0^*,\PP_1^*)\]
\end{proof}

Furthermore, notice that because the dual problem maximizes a concave functional over a convex set, the set of maximizers of $\dl$ is convex.

\subsection{Proof of Theorem~\ref{th:dual_regularity}}

Theorem~\ref{th:dual_regularity} rests on the following result:
\begin{theorem}[\citep{ChampionDePascaleJuutinen07}]\label{th:inf_cyclical_monotonicity}
    Let $\nu,\rho$ be two compactly supported Borel measures with the same mass. Assume that $\nu\ll \rho$. 
    Then $\rho=\nu\circ T^{-1}$ for some  Borel function $T\colon \Rset^d\to \Rset^d$ that satisfies $\|T(\bx)-\bx\|\leq \e$ $\mu$-a.e.
\end{theorem}
This theorem is a consequence of Theorem~5.5 of~\citep{ChampionDePascaleJuutinen07}.

Next we notice that if $\nu$ is compactly supported and $\rho\in \Wball \e (\nu)$, then $\rho$ is compactly supported as well.
In fact, due to Lemma~\ref{lemma:W_inf_set_characterization}, the $W_\infty$-norm is intimately related to the $\empty^\e$ operation. We prove the following result in Appendix~\ref{app:W_infty}:


\begin{restatable}{lem}{lemmaWinfballsupports}\label{lemma:W_inf_ball_supports}
    Assume that $\rho\in \Wball \e(\nu)$. Then $\supp \rho \subset (\supp \nu )^\e$. 
    
\end{restatable}




We now prove Theorem~\ref{th:dual_regularity}.
\begin{proof}[Proof of Theorem~\ref{th:dual_regularity}]
    Let $\PP_0^*,\PP_1^*$ be maximizers of $\dl$ over $\Wball \e (\PP_0)\times \Wball \e(\PP_1)$. Then because $\PP_0,\PP_1$ are compactly supported, Lemma~\ref{lemma:W_inf_ball_supports} implies that $\PP_0^*$, $\PP_1^*$ are compactly supported as well. Therefore, by Theorem~\ref{th:inf_cyclical_monotonicity}, $\PP_0^*=\PP_0\circ T_0^{-1}$, $\PP_1^*=\PP_1\circ T_1^{-1}$, where $T_i\colon \Rset^d\to \Rset^d$ are functions with $\|T(\bx)-\bx\|\leq \e$ $\mu$-a.e. 
\end{proof}
